FormalMATH: Benchmarking Formal Mathematical Reasoning of Large Language Models

Formal mathematical reasoning remains a critical challenge for artificial intelligence, hindered by limitations of existing benchmarks in scope and scale. To address this, we present FormalMATH, a large-scale Lean4 benchmark comprising 5,560 formally verified problems spanning from high-school Olympiad challenges to undergraduate-level theorems across diverse domains (e.g., algebra, applied mathematics, calculus, number theory, and discrete mathematics). To mitigate the inefficiency of manual formalization, we introduce a novel human-in-the-loop autoformalization pipeline that integrates: (1) specialized large language models (LLMs) for statement autoformalization, (2) multi-LLM semantic verification, and (3) negation-based disproof filtering strategies using off-the-shelf LLM-based provers. This approach reduces expert annotation costs by retaining 72.09% of statements before manual verification while ensuring fidelity to the original natural-language problems. Our evaluation of state-of-the-art LLM-based theorem provers reveals significant limitations: even the strongest models achieve only 16.46% success rate under practical sampling budgets, exhibiting pronounced domain bias (e.g., excelling in algebra but failing in calculus) and over-reliance on simplified automation tactics. Notably, we identify a counterintuitive inverse relationship between natural-language solution guidance and proof success in chain-of-thought reasoning scenarios, suggesting that human-written informal reasoning introduces noise rather than clarity in the formal reasoning settings. We believe that FormalMATH provides a robust benchmark for benchmarking formal mathematical reasoning.

==> contents/abstract.tex <==
\begin{abstract}
Formal mathematical reasoning is a cornerstone of human intelligence and remains an open challenge for AI systems. 
Progress is hindered by existing benchmarks in scope and scale.
We introduce FormalMATH, a large-scale Lean4 benchmark comprising 5,560 formally verified mathematical statements spanning diverse domains (algebra, statistics, calculus, number theory, and discrete mathematics, integral, and differentiation, etc) and difficulty levels (from high-school olympiads to undergraduate theorems). 
To address inefficiencies in manual formalization, we propose a human-in-the-loop pipeline integrating autoformalization (through specialized language models) and automated verification (through multi-LLM semantics verification and negation-based disproof via off-the-shelf LLM-based provers), significantly reducing annotation costs. 
Evaluations of state-of-the-art provers reveal critical limitations, such as persistent domain bias toward high-school-level algebra and applied mathematics, reliance on automated tactics, and ineffectiveness of natural language solution guidance. 
FormalMATH provides a robust benchmark for advancing automated formal reasoning and identifying critical weaknesses in current systems.

\end{abstract}


==> contents/exp.tex <==
\section{Evaluating Formal Theorem Prover LLMs on FormalMATH}
\label{exp}
\begin{table}[!t]
\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{0pt}
\setlength{\tabcolsep}{18pt}
\renewcommand{\arraystretch}{1.1}
\small
\centering
    \begin{tabular}{lcc}
        \textbf{Method}  & \textbf{Sampling budget} & \textbf{Pass@$K$ (\%)} \\
        \shline
        \multicolumn{3}{c}{\textit{Best-First Tree Search Methods}} \\[0.5mm]
        \multirow{5}{*}{BFS(DeepSeek-V1.5-RL) \cite{xin2024deepseek}}
        &$1\times32\times100$&  $4.91$ \\
        &$4\times32\times100$&  $10.29$ \\
        &$8\times32\times100$&  $12.16$ \\
        &$16\times32\times100$&  $14.96$ \\
        &$32\times32\times100$&  $17.41$ \\
        \hline
        \multirow{5}{*}{BFS(InternLM-V2.5) \cite{wu2024internlm2}}
        &$1\times32\times100$&  $7.87$ \\
        &$4\times32\times100$&  $15.79$ \\
        &$8\times32\times100$&  $20.02$ \\
        &$16\times32\times100$&  $22.74$ \\
        &$32\times32\times100$&  $25.65$ \\
        \hline
        \multirow{5}{*}{BFS(BFS-Prover) \cite{xin2025bfs}}
        &$1\times32\times100$&  $27.10$ \\
        &$4\times32\times100$&  $34.04$ \\
        &$8\times32\times100$&  $37.56$ \\
        &$16\times32\times100$&  $41.75$ \\
        &$32\times32\times100$&  $45.88$ \\
        \shline
        \multicolumn{3}{c}{\textit{Single-Pass Generation Methods}} \\[0.5mm]
        Kimina-Prover-7B~\cite{wang2025kiminaproverpreviewlargeformal} & 32 & $48.94$ \\
        \hline
        \multirow{6}{*}{STP~\cite{dong2025beyond}}
        &32&  $48.59$ \\
        &128&  $50.35$ \\
        &512&  $51.45$ \\
        &1024&  $52.03$ \\
        &2048&  $52.60$ \\
        &3200&  $53.17$ \\
        \hline
        \multirow{6}{*}{DeepSeek-V1.5-SFT~\cite{xin2024deepseek}}
        &$32$&  $40.40$ \\
        &128&  $42.11$ \\
        &512&  $44.17$ \\
        &1024&  $45.08$ \\
        &2048&  $46.12$ \\
        &3200&  $46.82$ \\
        \hline
        \multirow{6}{*}{DeepSeek-V1.5-RL~\cite{xin2024deepseek}}
        &32&  $47.98$ \\
        &128&  $48.75$ \\
        &512&  $49.27$ \\
        &1024&  $49.68$ \\
        &2048&  $50.08$ \\
        &3200&  $50.35$ \\
        \hline
        \multirow{6}{*}{Goedel-Prover~\cite{lin2025goedel}}
        &32&  $46.70$ \\
        &128&  $48.02$ \\
        &512&  $48.68$ \\
        &1024&  $49.04$ \\
        &2048&  $49.20$ \\
        &3200&  $49.41$ \\
        \hline
        \multirow{1}{*}{Ensemble System} &$4\times3200$&54.11 \\

    \end{tabular}    
    \caption{\small Performance comparison of theorem prover LLMs on FormalMATH-Lite.}
    \label{tab:main-results}
    \vspace{-1mm}
\end{table}


\subsection{Experimental Setup}
\noindent \textbf{Models.} 
In this section, we conduct a comprehensive evaluation of existing open-source LLM-based provers, focusing on two distinct proof-generation approaches: 
\vspace{1.5mm}
\begin{itemize}[leftmargin=*,nosep]
\setlength\itemsep{0.42em}
\item Best-First-Tree-search-based methods (BFS), where each node in the search tree represents an intermediate proof state. The base models include: BFS-Prover~\cite{xin2025bfs}, DeepSeek-Prover-V1.5-RL~\cite{xin2024deepseek}, and InternLM-V2.5-Prover~\cite{wu2024internlm2}. 
\item Single-pass generation methods (SPG), which directly produce the entire proof without iterative refinement or intermediate steps. The base models include: STP~\cite{dong2025beyond}, DeepSeek-Prover-V1.5-SFT and DeepSeek-Prover-V1.5-RL~\cite{xin2024deepseek}, Goedel-Prover~\cite{lin2025goedel}, and Kimina-Prover-7B~\cite{wang2025kiminaproverpreviewlargeformal}.
\end{itemize}

\vspace{1.5mm}

\noindent \textbf{Metric.} 
We evaluate performance using the pass@$K$, which measures whether a model produces at least one valid proof within $K$ attempts. 
The definition of $K$ depends on the proof-generation approach: (1) BFS-based methods: $K = N \times S \times T$, where $N$ denotes the number of best-first-search attempts, $S$ denotes the number of tactics generated during each expansion, and $T$ is the number of expansion iterations; (2) Single-pass generation methods: $K$ is the number of proofs sampled from the model.

\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \setlength{\abovecaptionskip}{4pt}
  \setlength{\belowcaptionskip}{5pt}
  \includegraphics[width=0.5\textwidth]{contents/images/verifier.pdf}
  \caption{\small Our efficient verifier implementation.}
  \label{fig:tree_verifier}
\end{wrapfigure}

\vspace{1.5mm}

\noindent \textbf{Verifier.} 
In Lean4, the correctness of proofs is verified by the compiler~\cite{repl}. 
However, verifying individual proofs is often time-consuming, largely due to the significant overhead associated with importing the Mathlib4 library~\cite{mathlib}. 
To mitigate this inefficiency, we use a tree-structured parallelism approach (see Figure~\ref{fig:tree_verifier}).
In this implementation, a parent thread manages the root node, which handles the computationally intensive import operations of Mathlib4. 
Concurrently, child threads process subsequent nodes in parallel, each corresponding to an individual proof. 
By centralizing the costly import operation at the root, redundant overhead is eliminated, and resources are efficiently allocated to parallelize proof verification.
This simple trick effectively optimizes test-time efficiency by avoiding repeated computational overhead, ensuring scalable and efficient utilization of computational resources.

\begin{figure}[tbp]
  \centering
  \setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{5pt}
  \includegraphics[width=1\textwidth]{contents/images/radar-custom_v2.pdf}
  \caption{\small Breakdown of accuracy by mathematical domain within FormalMATH.} 
  \label{fig:category_result}
\end{figure}

\vspace{1mm}
\noindent \textbf{Prompts.}
Unless otherwise specified, all experiments use vanilla generation strategies (see Example~\ref{textbox:prompt_vanilla}) as the default approach, where models directly generate Lean4 proof code without explicit chain-of-thought (CoT) rationales or natural language explanations.
To systematically evaluate the impact of structured reasoning guidance, we implement two prompting variants: (1) Simple CoT prompting (see Example~\ref{textbox:prompt_cot}) which requires models to interleave natural language reasoning steps with formal Lean4 proof tactics, and (2) NL-augmented CoT: natural language solution-augmented prompting (see Example~\ref{textbox:prompt_nat}) which enhances CoT with human-written mathematical solution sketches.


\begin{figure}[tbp]
  \centering
  \vspace{-1mm}
  \setlength{\belowcaptionskip}{0pt}
  \captionsetup[subfigure]{belowskip=-5pt, aboveskip=2.5pt}
  \captionsetup[subfigure]{margin=25pt}
  \begin{subfigure}[b]{0.49\textwidth}
    \centering

    \includegraphics[width=\textwidth]{contents/images/bingtu.pdf}
    \caption{\small Training domains of Goedel-Prover}
    \label{fig:godel_pie}
  \end{subfigure}
  \hfill 
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/images/ppl_dpsk_sft.pdf}
    \caption{\small Perplexity of DeepSeek-V1.5-SFT}
    \label{ppl}
  \end{subfigure}
  \caption{\small (a) The mathematical domain distribution of Goedel-Prover's training dataset. (b) The perplexity distribution of Deepseek-V1.5-SFT across various proof generation modes.}
  \label{fig:ppl}
\end{figure}




\subsection{Experimental Results and Discussions}
\noindent \textbf{Existing Provers Demonstrate Limited Performance on FormalMATH.} 
Existing LLM-based theorem provers perform poorly on the FormalMATH under constrained computational budgets (See Figure~\ref{fig:main:sota}), with the best single-pass generation approaches and BFS-based strategies attaining only 16.46\% and 11.13\% accuracy, respectively, under comparable sampling constraints (\ie, 32 trials for single-pass versus $1\times32\times100$ expansions for BFS-based methods). 
Kimina-Prover-7B, the best single-pass model that leverages distillation fine-tuning on the reasoning traces generated by Kimina-Prover-72B, outperforms BFS-Prover. Both provers employ Qwen2.5-Math-7B as the base model, and BFS-Prover uses an extensive post-training strategy (\ie, SFT and DPO~\cite{rafailov2023direct}).
This performance gap becomes more pronounced for Deepseek-V1.5-RL, which achieves 10.18\% through single-pass generation. In contrast, its BFS-enhanced counterpart achieves 1.19\% success rate.
These results suggest that the BFS strategy may not yield practical benefits under modest sampling budgets, potentially due to the inefficient exploration-exploitation tradeoffs in complex theorem spaces.



\vspace{1.5mm}

\noindent \textbf{Performance of Test-Time Compute Scaling on FormalMATH.}
Table~\ref{tab:main-results} reveals diminishing returns in formal theorem proving. Specifically, STP gains only 4.58\% (from 48.59\% by Pass@32 to 53.17\% by Pass@3200) with a 100$\times$ sampling budget increase, while BFS-Prover shows stronger scaling potential with a 18.78\% gain under an expanded search (via 32$\times$ sampling budget increase). 
Moreover, ensembling all single-pass methods yields a marginal 0.84\% improvement (From 53.17\% by STP to 54.11\% by the ensemble). This is in sharp contrast to the near-linear scaling performance increments in informal reasoning~\cite{muennighoff2025s1}.
In informal mathematics, pseudo-continuous reward signals during sampling create pathways where imperfect reasoning chains, despite their logical flaws, can occasionally "stumble" into correct answers. This suggests that valid conclusions may emerge even when the intermediate steps aren't rigorously sound.
However, formal theorem proving lacks this tolerance. For example, a single misplaced tactic or type error can invalidate the entire proof trajectory, making the correct conclusion unreachable.
While hybrid neuro-symbolic methods (\eg, verifier-guided search) show theoretical promises, current BFS approaches demand impractical computational budgets compared to single-pass generation methods.

\begin{figure}[tbp]
  \centering
  \vspace{-1mm}
  \setlength{\belowcaptionskip}{0pt}
  \captionsetup[subfigure]{belowskip=-6pt, aboveskip=2pt}
  \captionsetup[subfigure]{margin=25pt}
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/images/TTS-SFT.pdf}
    \caption{\small DeepSeek-V1.5-SFT}
    \label{a}
  \end{subfigure}
  \hfill 
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/images/TTS-RL.pdf}
    \caption{\small DeepSeek-V1.5-RL}
    \label{b}
  \end{subfigure}
  \caption{\small Pass@K accuracy curves for DeepSeek‑V1.5 provers across different reasoning configurations.}
  \label{fig:tts}
\end{figure}

\noindent \textbf{Provers' Unbalanced Performance Across Mathematical Domains of FormalMATH.}
Figure~\ref{fig:category_result} reveals a significant domain bias in existing theorem provers. 
Under Pass@32, Godel-Prover achieves high success rates in algebra-related domains (\eg, 17.47\% in high school algebra, 50\% in undergraduate algebra) but struggles in calculus (5.21\%), and discrete mathematics (0\%). This pattern persists at the undergraduate level, where precalculus (33.71\%) outperforms differentiation (1.92\%) and integration (0\%).
Such a domain bias is likely due to the biased training data. 
We adopt the same domain categorization of FormalMATH to inspect the training data of Godel-Prover. We randomly sample 200 problems, and the domain distribution shown in the Figure~\ref{fig:godel_pie}, where the mathematical domain of its training data is heavily biased toward applied mathematics and algebra, which account for 68\% of the dataset, while discrete math, number theory, and precalculus account for less than 5\%.

\vspace{1.5mm}
\noindent \textbf{CoT Enhances Model Capabilities on FormalMATH.}
We evaluate three different reasoning strategies in Lean4 proof generations: (1) simple CoT prompting, (2) NL-augmented CoT: CoT augmented with natural language solution example, and (3) vanilla generation strategies via test-time scaling on FormalMATH-Lite (See Figure~\ref{fig:tts}).
Our goal is to \textit{measure whether--and to what extent--informal mathematical reasoning contributes to the rigor and effectiveness of subsequently derived formal proofs.}.

\vspace{1mm}

\noindent Across both SFT and RL configurations, we observe a consistent ranking of decoding strategies. Generally, simple CoT attains the highest Pass@K (from K equals 32 to 3200) accuracy, while NL-augmented CoT performs an intermediate position better than vanilla decoding.
For example, under $K=3200$, DeepSeek‑V1.5-SFT achieves 50.6\% with CoT and 49.2\% with NL‑augmented CoT and 47.0\% with vanilla decoding, and DeepSeek‑V1.5-RL achieves 51.7\%,  51.2\%, and 49.8\%, respectively.
On the other hand, it appears to be counterintuitive that NL-augmented CoT does not yield superior results compared to simple CoT. 
The perplexity distribution for each mode in Figure~\ref{ppl} shows a counterintuitive phenomenon, where incorporating NL solutions tends to increase perplexity across a broad range of Lean4 problems.

\vspace{1mm}
\begin{tcolorbox}[
    title=\textbf{\scriptsize  The solution strategy provided by the prover is specific enough.},
    colframe=c3,
    colback=c4!5,
    boxrule=0.5pt,
    fonttitle=\scriptsize, %
    fontupper=\scriptsize, %
     breakable
]
\footnotesize
\vspace{0.2em}
\textbf{\scriptsize CoT (Success):}
\begin{lstlisting}[frame=single, basicstyle=\scriptsize]
theorem algebra_68653_cot : ¬ ∃ x y : ℤ, x^3 + y^4 = 7 := by
  -- Assume there are integers x and y such that x^3 + y^4 = 7.
  intro h
  -- Extract the integers x and y from the assumption.
  rcases h with ⟨x, y, hxy⟩
  -- Consider the equation modulo 13.
  have hxy_mod : (x^3 + y^4) %
  -- Calculate the possible values of x^3 modulo 13.
  have x3_mod : x^3 %
    have : x %
    rcases this with (h | h | h | h | h | h | h | h | h | h | h | h | h) <;> simp [h, pow_succ, Int.mul_emod]
  -- Calculate the possible values of y^4 modulo 13.
  have y4_mod : y^4 %
    have : y %
    rcases this with (h | h | h | h | h | h | h | h | h | h | h | h | h) <;> simp [h, pow_succ, Int.mul_emod]
  -- Check that x^3 + y^4 cannot be congruent to 7 modulo 13.
  rcases x3_mod with (h1 | h1 | h1 | h1 | h1) <;> rcases y4_mod with (h2 | h2 | h2 | h2) <;> simp [h1, h2, Int.add_emod] at hxy_mod <;> omega

\end{lstlisting}
\par
\vspace{0.1\baselineskip}
\textbf{\scriptsize NL-agumented CoT (Not Success):} 

\lstset{
    frame=single,
    basicstyle=\scriptsize,
    xleftmargin=0.1pt,
    framexleftmargin=0.1pt,
    keywordstyle=\bfseries,
    morecomment=[l]{--},   %
    commentstyle=\color{gray}, 
    escapeinside={@!}{@!},     %
     moredelim=**[is][\color{red}]{@}{@},
     language=lean,
}

\begin{lstlisting}[frame=single, basicstyle=\scriptsize]
theorem algebra_68653_nat : ¬ ∃ x y : ℤ, x^3 + y^4 = 7 := by   /-
  We aim to show that there do not exist integers \( x \) and \( y \) such that \( x^3 + y^4 = 7 \). Suppose, for the sake of contradiction, that such integers exist. We would then have \( x^3 + y^4 = 7 \). We analyze the possible values of \( x^3 \mod 7 \) and \( y^4 \mod 7 \) to find a contradiction.
  1. **Lemma:** For any integer \( x \), \( x^3 \mod 7 \) can only be 0, 1, or -1.
     - Proof: By examining all possible values of \( x \mod 7 \), we find that \( x^3 \mod 7 \) is either 0, 1, or -1.
  2. **Lemma:** For any integer \( y \), \( y^4 \mod 7 \) can only be 0, 1, or 2.
     - Proof: By examining all possible values of \( y \mod 7 \), we find that \( y^4 \mod 7 \) is either 0, 1, or 2.
  3. **Combining the Lemmas:** If \( x^3 + y^4 = 7 \), then \( x^3 \mod 7 \) and \( y^4 \mod 7 \) must sum to 7 modulo 7. However, the possible values of \( x^3 \mod 7 \) are 0, 1, or -1, and the possible values of \( y^4 \mod 7 \) are 0, 1, or 2. None of these combinations can sum to 7 modulo 7, leading to a contradiction.
  Thus, we conclude that there do not exist integers \( x \) and \( y \) such that \( x^3 + y^4 = 7 \).
  -/
  -- Assume for contradiction that there exist integers x and y such that x^3 + y^4 = 7.
  intro h
  obtain ⟨x, y, hxy⟩ := h
  -- Analyze the possible values of x^3 modulo 7.
  have hx : x^3 %
    have hx : x %
      omega
    rcases hx with (h | h | h | h | h | h | h) <;>
      simp [h, pow_three, Int.mul_emod, Int.add_emod]
  -- Analyze the possible values of y^4 modulo 7.
  have hy : y^4 %
    have hy : y %
      omega
    rcases hy with (h | h | h | h | h | h | h) <;>
      simp [h, pow_four, Int.mul_emod, Int.add_emod]
  -- Combine the results to find a contradiction.
  have h7 : (x^3 + y^4) %
    rcases hx with (h | h | h) <;>
      rcases hy with (h' | h' | h') <;>
        simp [h, h', Int.add_emod, Int.mul_emod]
  -- Conclude the proof by contradiction.
  @!\colorbox{c1}{omega}@!
\end{lstlisting}
\par
\vspace{0.1\baselineskip}
\textbf{\scriptsize Vanilla (Not Success):} 

\lstset{
    frame=single,
    basicstyle=\scriptsize,
    xleftmargin=0.1pt,
    framexleftmargin=0.1pt,
    keywordstyle=\bfseries,
    morecomment=[l]{--},   %
    commentstyle=\color{gray}, 
    escapeinside={@!}{@!},     %
     moredelim=**[is][\color{red}]{@}{@},
     language=lean,
}

\begin{lstlisting}[frame=single, basicstyle=\scriptsize]
theorem algebra_68653_vanilla : ¬ ∃ x y : ℤ, x^3 + y^4 = 7 := by
  intro h; rcases h with ⟨x, y, hxy⟩; have hx : x^3 ≥ 0 := by positivity; have hy : y^4 ≥ 0 := by positivity
  @!\colorbox{c1}{linarith}@!
\end{lstlisting}
\scriptsize
\label{textbox:dpsk_cot}
\end{tcolorbox}


\noindent In Example~\ref{textbox:dpsk_cot}, the failed NL‑augmented CoT proof reveals a fundamental error pattern: although the natural‑language outline and the Lean4 script target the same semantic goal, the high‑level sketch omits essential parameters and case distinctions that Lean’s tactics require. 
We hypothesize that this discrepancy stems from an intrinsic misalignment between the action space of informal, natural‑language reasoning and the tactic space of Lean4 formalization.

\vspace{1mm}

\noindent In this particular instance, the NL‑augmented CoT followed the NL solution by working on \texttt{modulo 7}, and asserting informally that $x^3 \; mod \;7 \in \{0,1,6\}$ and $y^4 \;mod\; 7\;\in \{0,1,2\}$ but does not materializes those assertions into the fifteen concrete \texttt{have $_{ \dots} =$ const} hypotheses branch that Lean4's decision procedures demand.
As a result, when the script invokes tactics (\ie, \texttt{omega}) reports the context simply lacks the linear congruences needed to derive a contradiction.

\vspace{1mm}


\noindent In contrast, simple CoT autonomously selects the larger prime modulus 13 without human written prior, interleaves each residue‐case split with explicit tactic calls producing hypotheses like \texttt{have h : $x^3$ \% 13 = 5 := by simp [hxy\_mod]},
and then immediately discharges each branch with $\texttt{omega}$.
By reconstructing its own detailed, tactic‐level proof, CoT aligns semantic insight with low‑level proof obligations, guaranteeing that every subgoal carries the precise numeric constraints required for full automation--whereas the NL‑augmented approach, despite being semantically correct at a high level, leaves critical tactical steps unstated and thus fails to complete the proof.






==> lstlean.tex <==

\lstdefinelanguage{lean} {

mathescape=true,
texcl=false,

morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, while,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes, opaque,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

morekeywords=[2]{Sort, Type, Prop},

morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},


literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 %

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1
{|}{\ensuremath{\mid}}1,

morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

showstringspaces=false,

keepspaces=true,

morestring=[b]",
morestring=[d],

tabsize=3,

extendedchars=true,

sensitive=true,

breaklines=true,
breakatwhitespace=true,

basicstyle=\ttfamily\small,

captionpos=b,

columns=[l]fullflexible,


identifierstyle={\ttfamily\color{black}},

keywordstyle=[1]{\ttfamily\color{keywordcolor}},

keywordstyle=[2]{\ttfamily\color{sortcolor}},

keywordstyle=[3]{\ttfamily\color{tacticcolor}},

keywordstyle=[4]{\ttfamily\color{attributecolor}},

stringstyle=\ttfamily,

commentstyle={\ttfamily\footnotesize },

}


==> map_resource/math_macro.tex <==
\newcommand{\seedmoe}{Seed-MoE}


==> map_resource/packages.tex <==
\usepackage{natbib}

\usepackage{CJKutf8}

\usepackage{xargs}  

\usepackage{todonotes}  

\usepackage{multirow}


\usepackage{cleveref}

\usepackage{amsmath}
\usepackage{dsfont}



\usepackage{subcaption}


\usepackage{svg}
\usepackage{fullpage}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\synctex=-1
\usepackage{fix-cm}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{booktabs} 
\usepackage{caption}
\usepackage{subcaption}
\usepackage{comment}
\usepackage{microtype} 
\usepackage{verbatim}
\usepackage[square,sort,comma,numbers]{natbib}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{graphics}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{enumerate}
\usepackage[dvipsnames]{xcolor}
\definecolor{Gray}{gray}{0.96}
\usepackage[align=center,shadow=true,shadowsize=6pt,nobreak=true,framemethod=tikz,skipabove=9.5pt,skipbelow=9pt,innertopmargin=5pt,innerbottommargin=5pt,innerleftmargin=5pt,innerrightmargin=5pt,leftmargin=1.5pt,rightmargin=1.5pt]{mdframed}
\usetikzlibrary{shadows}
\usepackage{tcolorbox}
\renewcommand{\captionlabelfont}{\small}
\makeatletter
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
\theoremstyle{plain}
\newtheorem{lemma}{\protect\lemmaname}
\newtheorem{corollary}{\protect\corollaryname}
\newtheorem{remark}{\protect\remarkname}
\theoremstyle{remark}
\newtheorem*{rem*}{\protect\remarkname}
\newtheorem{assumption}{\protect\assumptionname}
\theoremstyle{plain}
\newtheorem{manualtheoreminner}{Theorem}
\newenvironment{manualtheorem}[1]{%
  \renewcommand\themanualtheoreminner{#1}%
  \manualtheoreminner
}{\endmanualtheoreminner}

\@ifundefined{date}{}{\date{}}
\usepackage{color}
\usepackage{colortbl}
\usepackage{svg}
\usepackage[lined,boxed,ruled, linesnumbered, algo2e]{algorithm2e}

\usepackage[tmargin=.9in, lmargin=.8in, rmargin=.8in, bmargin=.9in]
           {geometry}

\usepackage{amsfonts}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{wrapfig}
\allowdisplaybreaks

\usepackage{multicol}



\usepackage{xcolor}
\input{math_commands.tex}
\usepackage{svg}
\usepackage{url}
\usepackage{graphicx}
\usepackage{colortbl}
\usepackage{longtable}
\usepackage{array}
\usepackage{booktabs}
\usepackage{wrapfig}
\usepackage{mdframed,lipsum}
\usepackage{multirow}
\usepackage{bbding}
\definecolor{darkblue}{RGB}{25, 50, 112}
\definecolor{c1}{HTML}{fdb4ae}
\definecolor{c2}{HTML}{731d1e}

\usepackage[pagebackref=true,breaklinks=true,colorlinks=true,bookmarks=false]{hyperref}
\definecolor{deepred}{HTML}{940000}
\definecolor{green2}{HTML}{BFF6BA}
\hypersetup{linkcolor=deepred}
\hypersetup{urlcolor  = [rgb]{0.4,0.15,0.95}}
\hypersetup{citecolor=[rgb]{0.4,0.15,0.95}}
\usepackage{tabularx} %
\usepackage{listings} %
\usepackage{cleveref}

\usepackage{pifont}
\usepackage{tocloft}
\usepackage[toc,page,header]{appendix}
\usepackage{adjustbox}
\usepackage{minitoc}
\renewcommand{\ptifont}{\large \bf}
\renewcommand \thepart{}
\renewcommand \partname{}


\definecolor{keywordcolor}{rgb}{0.7, 0.1, 0.1}   %
\definecolor{tacticcolor}{rgb}{0.0, 0.1, 0.6}    %
\definecolor{commentcolor}{rgb}{0.4, 0.4, 0.4}   %
\definecolor{symbolcolor}{rgb}{0.0, 0.1, 0.6}    %
\definecolor{sortcolor}{rgb}{0.1, 0.5, 0.1}      %
\definecolor{attributecolor}{rgb}{0.7, 0.1, 0.1} %
\usepackage{listings}
\def\lstlanguagefiles{lstlean.tex}


\lstset{
    inputencoding=utf8,
    extendedchars=true,       
    language=lean,
    moredelim=[is][\colorbox{yellow}]{「}{」},
}


\newcommand{\lightblue}[1]{\definecolor{lightblue}{rgb}{0.68, 0.85, 0.9}\colorbox{lightblue}{#1}}
\lstnewenvironment{pythoncode}[1][]{
  \lstset{
    language=Python,
    basicstyle=\small\ttfamily,
    numbers=left,
    numberstyle=\tiny,
    stepnumber=1,
    numbersep=5pt,
    frame=single,
    showstringspaces=false,
    keywordstyle=\color{blue},
    commentstyle=\color{gray},
    stringstyle=\color{purple},
    captionpos=b,
    breaklines=true,
    breakatwhitespace=true,
    tabsize=4,
    caption=#1
  }
}{}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\our}{FormalMATH}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth
  \global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}

